Evidence of high-mass star formation through multi-scale mass accretion in hub-filament-system clouds

We present a statistical study of a sample of 17 hub-filament-system (HFS) clouds of high-mass star formation using high-angular resolution ($\sim$1-2 arcsecond) ALMA 1.3mm and 3mm continuum data. The sample includes 8 infrared (IR)-dark and 9 IR-bright types, which correspond to an evolutionary sequence from the IR-dark to IR-bright stage. The central massive clumps and their associated most massive cores are observed to follow a trend of increasing mass ($M$) and mass surface density ($\Sigma$) with evolution from IR-dark to IR-bright stage. In addition, a mass-segregated cluster of young stellar objects (YSOs) are revealed in both IR-dark and IR-bright HFSs with massive YSOs located in the hub and the population of low-mass YSOs distributed over larger areas. Moreover, outflow feedback in all HFSs are found to escape preferentially through the inter-filamentary diffuse cavities, suggesting that outflows would render a limited effect on the disruption of the HFSs and ongoing high-mass star formation therein. From the above observations, we suggest that high-mass star formation in the HFSs can be described by a multi-scale mass accretion/transfer scenario, from hub-composing filaments through clumps down to cores, that can naturally lead to a mass-segregated cluster of stars.

==> bbl.tex <==
\begin{thebibliography}{}
\makeatletter
\relax
\def\mn@urlcharsother{\let\do\@makeother \do\$\do\&\do\#\do\^\do\_\do\%\do\~}
\def\mn@doi{\begingroup\mn@urlcharsother \@ifnextchar [ {\mn@doi@}
  {\mn@doi@[]}}
\def\mn@doi@[#1]#2{\def\@tempa{#1}\ifx\@tempa\@empty \href
  {http://dx.doi.org/#2} {doi:#2}\else \href {http://dx.doi.org/#2} {#1}\fi
  \endgroup}
\def\mn@eprint#1#2{\mn@eprint@#1:#2::\@nil}
\def\mn@eprint@arXiv#1{\href {http://arxiv.org/abs/#1} {{\tt arXiv:#1}}}
\def\mn@eprint@dblp#1{\href {http://dblp.uni-trier.de/rec/bibtex/#1.xml}
  {dblp:#1}}
\def\mn@eprint@#1:#2:#3:#4\@nil{\def\@tempa {#1}\def\@tempb {#2}\def\@tempc
  {#3}\ifx \@tempc \@empty \let \@tempc \@tempb \let \@tempb \@tempa \fi \ifx
  \@tempb \@empty \def\@tempb {arXiv}\fi \@ifundefined
  {mn@eprint@\@tempb}{\@tempb:\@tempc}{\expandafter \expandafter \csname
  mn@eprint@\@tempb\endcsname \expandafter{\@tempc}}}

\makeatother

\bibitem[\protect\citeauthoryear{Anderson et al.}{2021}]{And21} Anderson M., Peretto N., Ragan S.~E., Rigby A.~J., Avison A., Duarte-Cabral A., Fuller G.~A., et al., 2021, MNRAS, 508, 2964. doi:10.1093/mnras/stab2674
\bibitem[\protect\citeauthoryear{Andr{\'e} et al.}{2010}]{And10} Andr{\'e} P., Men'shchikov A., Bontemps S., K{\"o}nyves V., Motte F., Schneider N., Didelon P., et al., 2010, A\&A, 518, L102. doi:10.1051/0004-6361/201014666
\bibitem[\protect\citeauthoryear{Andr{\'e} et al.}{2019}]{And19} Andr{\'e} P., Arzoumanian D., K{\"o}nyves V., Shimajiri Y., Palmeirim P., 2019, A\&A, 629, L4. doi:10.1051/0004-6361/201935915
\bibitem[\protect\citeauthoryear{Anathpindika \& Whitworth}{2008}]{Ana08} Anathpindika S., Whitworth A.~P., 2008, A\&A, 487, 605. doi:10.1051/0004-6361:200810308
\bibitem[\protect\citeauthoryear{Astropy Collaboration et al.}{2018}]{Ast18} Astropy Collaboration, Price-Whelan A.~M., Sip{\H{o}}cz B.~M., G{\"u}nther H.~M., Lim P.~L., Crawford S.~M., Conseil S., et al., 2018, AJ, 156, 123. doi:10.3847/1538-3881/aabc4f
\bibitem[\protect\citeauthoryear{Bate}{2009}]{Bat09} Bate M.~R., 2009, MNRAS, 392, 1363. doi:10.1111/j.1365-2966.2008.14165.x
\bibitem[\protect\citeauthoryear{Bate}{2012}]{Bat12} Bate M.~R., 2012, MNRAS, 419, 3115. doi:10.1111/j.1365-2966.2011.19955.x
\bibitem[\protect\citeauthoryear{Baug et al.}{2021}]{Bau20} Baug T., Wang K., Liu T., Wu Y.-F., Li D., Zhang Q., Tang M., et al., 2021, MNRAS, 507, 4316. doi:10.1093/mnras/stab1902
\bibitem[\protect\citeauthoryear{Beltr{\'a}n et al.}{2022}]{Bel22} Beltr{\'a}n M.~T., Rivilla V.~M., Kumar M.~S.~N., Cesaroni R., Galli D., 2022, A\&A, 660, L4. doi:10.1051/0004-6361/202243361
\bibitem[\protect\citeauthoryear{Beuther et al.}{2018}]{Beu18} Beuther H., Mottram J.~C., Ahmadi A., Bosco F., Linz H., Henning T., Klaassen P., et al., 2018, A\&A, 617, A100. doi:10.1051/0004-6361/201833021
\bibitem[\protect\citeauthoryear{Bonnell et al.}{2001}]{Bon01} Bonnell I.~A., Bate M.~R., Clarke C.~J., Pringle J.~E., 2001, MNRAS, 323, 785. doi:10.1046/j.1365-8711.2001.04270.x
\bibitem[\protect\citeauthoryear{Bronfman, Nyman, \& May}{1996}]{Bro96} Bronfman L., Nyman L.-A., May J., 1996, A\&AS, 115, 81
\bibitem[\protect\citeauthoryear{Chen et al.}{2019}]{Che19} Chen H.-R.~V., Zhang Q., Wright M.~C.~H., Busquet G., Lin Y., Liu H.~B., Olguin F.~A., et al., 2019, ApJ, 875, 24. doi:10.3847/1538-4357/ab0f3e
\bibitem[\protect\citeauthoryear{Chevance et al.}{2022}]{Che22} Chevance M., Krumholz M.~R., McLeod A.~F., Ostriker E.~C., Rosolowsky E.~W., Sternberg A., 2022, arXiv, arXiv:2203.09570
\bibitem[\protect\citeauthoryear{Contreras et al.}{2013}]{Con13} Contreras Y., Schuller F., Urquhart J.~S., Csengeri T., Wyrowski F., Beuther H., Bontemps S., et al., 2013, A\&A, 549, A45. doi:10.1051/0004-6361/201220155
\bibitem[\protect\citeauthoryear{Dale \& Bonnell}{2011}]{Dal11} Dale J.~E., Bonnell I., 2011, MNRAS, 414, 321. doi:10.1111/j.1365-2966.2011.18392.x
\bibitem[\protect\citeauthoryear{Dunham et al.}{2008}]{Dun08} Dunham M.~M., Crapsi A., Evans N.~J., Bourke T.~L., Huard T.~L., Myers P.~C., Kauffmann J., 2008, ApJS, 179, 249. doi:10.1086/591085
\bibitem[\protect\citeauthoryear{Davis et al.}{2009}]{Dav09} Davis C.~J., Froebrich D., Stanke T., Megeath S.~T., Kumar M.~S.~N., Adamson A., Eisl{\"o}ffel J., et al., 2009, A\&A, 496, 153. doi:10.1051/0004-6361:200811096
\bibitem[\protect\citeauthoryear{Elia et al.}{2018}]{Eli18} Elia D., Strafella F., Dib S., Schneider N., Hennebelle P., Pezzuto S., Molinari S., et al., 2018, MNRAS, 481, 509. doi:10.1093/mnras/sty2170
\bibitem[\protect\citeauthoryear{Elia et al.}{2022}]{Eli22} Elia D., Molinari S., Schisano E., Soler J.~D., Merello M., Russeil D., Veneziani M., et al., 2022, arXiv, arXiv:2211.05573
\bibitem[\protect\citeauthoryear{Foster et al.}{2014}]{Fos14} Foster J.~B., Arce H.~G., Kassis M., Sanhueza P., Jackson J.~M., Finn S.~C., Offner S., et al., 2014, ApJ, 791, 108. doi:10.1088/0004-637X/791/2/108
\bibitem[\protect\citeauthoryear{Giannetti et al.}{2017}]{Gia17} Giannetti A., Leurini S., Wyrowski F., Urquhart J., Csengeri T., Menten K.~M., K{\"o}nig C., et al., 2017, A\&A, 603, A33. doi:10.1051/0004-6361/201630048
\bibitem[\protect\citeauthoryear{Ginsburg et al.}{2016}]{Gin16} Ginsburg A., Henkel C., Ao Y., Riquelme D., Kauffmann J., Pillai T., Mills E.~A.~C., et al., 2016, A\&A, 586, A50. doi:10.1051/0004-6361/201526100
\bibitem[\protect\citeauthoryear{Goodman, Pineda, \& Schnee}{2009}]{Goo09} Goodman A.~A., Pineda J.~E., Schnee S.~L., 2009, ApJ, 692, 91. doi:10.1088/0004-637X/692/1/91
\bibitem[\protect\citeauthoryear{Grudi{\'c} et al.}{2022}]{Gru22} Grudi{\'c} M.~Y., Guszejnov D., Offner S.~S.~R., Rosen A.~L., Raju A.~N., Faucher-Gigu{\`e}re C.-A., Hopkins P.~F., 2022, MNRAS, 512, 216. doi:10.1093/mnras/stac526
\bibitem[\protect\citeauthoryear{Guszejnov et al.}{2020}]{Gus20} Guszejnov D., Grudi{\'c} M.~Y., Hopkins P.~F., Offner S.~S.~R., Faucher-Gigu{\`e}re C.-A., 2020, MNRAS, 496, 5072. doi:10.1093/mnras/staa1883
\bibitem[\protect\citeauthoryear{Guszejnov et al.}{2021}]{Gus21} Guszejnov D., Grudi{\'c} M.~Y., Hopkins P.~F., Offner S.~S.~R., Faucher-Gigu{\`e}re C.-A., 2021, MNRAS, 502, 3646. doi:10.1093/mnras/stab278
\bibitem[\protect\citeauthoryear{Guo et al.}{2021}]{Guo21} Guo W., Chen X., Feng J., Sun L., Wang C., Su Y., Sun Y., et al., 2021, ApJ, 921, 23. doi:10.3847/1538-4357/ac15fe
\bibitem[\protect\citeauthoryear{Gutermuth \& Heyer}{2015}]{Gut15} Gutermuth R.~A., Heyer M., 2015, AJ, 149, 64. doi:10.1088/0004-6256/149/2/64
\bibitem[\protect\citeauthoryear{Guzm{\'a}n et al.}{2015}]{Guz15} Guzm{\'a}n A.~E., Sanhueza P., Contreras Y., Smith H.~A., Jackson J.~M., Hoq S., Rathborne J.~M., 2015, ApJ, 815, 130. doi:10.1088/0004-637X/815/2/130
\bibitem[\protect\citeauthoryear{Hacar et al.}{2022}]{Hac22} Hacar A., Clark S., Heitsch F., Kainulainen J., Panopoulou G., Seifried D., Smith R., 2022, arXiv, arXiv:2203.09562
\bibitem[\protect\citeauthoryear{Hennebelle et al.}{2020}]{Hen20} Hennebelle P., Commer{\c{c}}on B., Lee Y.-N., Chabrier G., 2020, ApJ, 904, 194. doi:10.3847/1538-4357/abbfab
\bibitem[\protect\citeauthoryear{Hennebelle et al.}{2022}]{Hen22} Hennebelle P., Lebreuilly U., Colman T., Elia D., Fuller G., Leurini S., Nony T., et al., 2022, arXiv, arXiv:2210.12475
\bibitem[\protect\citeauthoryear{Issac et al.}{2019}]{Iss19} Issac N., Tej A., Liu T., Varricatt W., Vig S., Ishwara Chandra C.~H., Schultheis M., 2019, MNRAS, 485, 1775. doi:10.1093/mnras/stz466
\bibitem[\protect\citeauthoryear{Krumholz \& Thompson}{2012}]{Kru12} Krumholz M.~R., Thompson T.~A., 2012, ApJ, 760, 155. doi:10.1088/0004-637X/760/2/155
\bibitem[\protect\citeauthoryear{Kuhn et al.}{2021}]{Kuh21} Kuhn M.~A., de Souza R.~S., Krone-Martins A., Castro-Ginard A., Ishida E.~E.~O., Povich M.~S., Hillenbrand L.~A., et al., 2021, ApJS, 254, 33. doi:10.3847/1538-4365/abe465
\bibitem[\protect\citeauthoryear{Kumar et al.}{2020}]{Kum20} Kumar M.~S.~N., Palmeirim P., Arzoumanian D., Inutsuka S.~I., 2020, A\&A, 642, A87. doi:10.1051/0004-6361/202038232
\bibitem[\protect\citeauthoryear{Kumar et al.}{2022}]{Kum22} Kumar M.~S.~N., Arzoumanian D., Men'shchikov A., Palmeirim P., Matsumura M., Inutsuka S., 2022, A\&A, 658, A114. doi:10.1051/0004-6361/202140363
\bibitem[\protect\citeauthoryear{Larson}{2003}]{Lar03} Larson R.~B., 2003, RPPh, 66, 1651. doi:10.1088/0034-4885/66/10/R03
\bibitem[\protect\citeauthoryear{Lee et al.}{2016}]{Lee16} Lee K.~I., Dunham M.~M., Myers P.~C., Arce H.~G., Bourke T.~L., Goodman A.~A., J{\o}rgensen J.~K., et al., 2016, ApJL, 820, L2. doi:10.3847/2041-8205/820/1/L2
\bibitem[\protect\citeauthoryear{Li et al.}{2020}]{Li 20} Li S., Sanhueza P., Zhang Q., Nakamura F., Lu X., Wang J., Liu T., et al., 2020, ApJ, 903, 119. doi:10.3847/1538-4357/abb81f
\bibitem[\protect\citeauthoryear{Li et al.}{2020b}]{Li 20b} Li S., Zhang Q., Liu H.~B., Beuther H., Palau A., Girart J.~M., Smith H., et al., 2020, ApJ, 896, 110. doi:10.3847/1538-4357/ab84f1
\bibitem[\protect\citeauthoryear{Li et al.}{2019}]{Li 19} Li S., Zhang Q., Pillai T., Stephens I.~W., Wang J., Li F., 2019, ApJ, 886, 130. doi:10.3847/1538-4357/ab464e
\bibitem[\protect\citeauthoryear{Liu et al.}{2012}]{Liu12} Liu H.~B., Quintana-Lacaci G., Wang K., Ho P.~T.~P., Li Z.-Y., Zhang Q., Zhang Z.-Y., 2012, ApJ, 745, 61. doi:10.1088/0004-637X/745/1/61
\bibitem[\protect\citeauthoryear{Liu et al.}{2015}]{Liu15} Liu H.~B., Galv{\'a}n-Madrid R., Jim{\'e}nez-Serra I., Rom{\'a}n-Z{\'u}{\~n}iga C., Zhang Q., Li Z., Chen H.-R., 2015, ApJ, 804, 37. doi:10.1088/0004-637X/804/1/37
\bibitem[\protect\citeauthoryear{Liu et al.}{2020}]{Liu20} Liu H.-L., Sanhueza P., Liu T., Zavagno A., Tang X.-D., Wu Y., Zhang S., 2020, ApJ, 901, 31. doi:10.3847/1538-4357/abadfe
\bibitem[\protect\citeauthoryear{Liu et al.}{2021}]{Liu21} Liu H.-L., Liu T., Evans N.~J., Wang K., Garay G., Qin S.-L., Li S., et al., 2021, MNRAS, 505, 2801. doi:10.1093/mnras/stab1352
\bibitem[\protect\citeauthoryear{Liu et al.}{2022a}]{Liu22a} Liu H.-L., Tej A., Liu T., Issac N., Saha A., Goldsmith P.~F., Wang J.-Z., et al., 2022a, MNRAS, 510, 5009. doi:10.1093/mnras/stab2757
\bibitem[\protect\citeauthoryear{Liu et al.}{2022b}]{Liu22b} Liu H.-L., Tej A., Liu T., Goldsmith P.~F., Stutz A., Juvela M., Qin S.-L., et al., 2022b, MNRAS, 511, 4480. doi:10.1093/mnras/stac378
\bibitem[\protect\citeauthoryear{Liu et al.}{2020a}]{Liu20a} Liu T., Evans N.~J., Kim K.-T., Goldsmith P.~F., Liu S.-Y., Zhang Q., Tatematsu K., et al., 2020a, MNRAS, 496, 2790. doi:10.1093/mnras/staa1577
\bibitem[\protect\citeauthoryear{Liu et al.}{2020b}]{Liu20b} Liu T., Evans N.~J., Kim K.-T., Goldsmith P.~F., Liu S.-Y., Zhang Q., Tatematsu K., et al., 2020b, MNRAS, 496, 2821. doi:10.1093/mnras/staa1501
\bibitem[\protect\citeauthoryear{Longmore et al.}{2014}]{Lon14} Longmore S.~N., Kruijssen J.~M.~D., Bastian N., Bally J., Rathborne J., Testi L., Stolte A., et al., 2014, prpl.conf, 291. doi:10.2458/azu\_uapress\_9780816531240-ch013
\bibitem[\protect\citeauthoryear{Louvet et al.}{2021}]{Lou21} Louvet F., Hennebelle P., Men'shchikov A., Didelon P., Ntormousi E., Motte F., 2021, A\&A, 653, A157. doi:10.1051/0004-6361/202040053
\bibitem[\protect\citeauthoryear{McKee \& Tan}{2003}]{McK03} McKee C.~F., Tan J.~C., 2003, ApJ, 585, 850. doi:10.1086/346149
\bibitem[\protect\citeauthoryear{Men'shchikov}{2021}]{Men21} Men'shchikov A., 2021, A\&A, 649, A89. doi:10.1051/0004-6361/202039913
\bibitem[\protect\citeauthoryear{Molinari et al.}{2010}]{Mol10} Molinari S., Swinyard B., Bally J., Barlow M., Bernard J.-P., Martin P., Moore T., et al., 2010, A\&A, 518, L100. doi:10.1051/0004-6361/201014659
\bibitem[\protect\citeauthoryear{Morii et al.}{2021}]{Mor21} Morii K., Sanhueza P., Nakamura F., Jackson J.~M., Li S., Beuther H., Zhang Q., et al., 2021, ApJ, 923, 147. doi:10.3847/1538-4357/ac2365
\bibitem[\protect\citeauthoryear{Motte et al.}{2022}]{Mot22} Motte F., Bontemps S., Csengeri T., Pouteau Y., Louvet F., Stutz A.~M., Cunningham N., et al., 2022, A\&A, 662, A8. doi:10.1051/0004-6361/202141677
\bibitem[\protect\citeauthoryear{Motte, Bontemps, \& Louvet}{2018}]{Mot18} Motte F., Bontemps S., Louvet F., 2018, ARA\&A, 56, 41. doi:10.1146/annurev-astro-091916-055235
\bibitem[\protect\citeauthoryear{Myers}{2009}]{Mye09} Myers P.~C., 2009, ApJ, 700, 1609. doi:10.1088/0004-637X/700/2/1609
\bibitem[\protect\citeauthoryear{Offner et al.}{2016}]{Off16} Offner S.~S.~R., Dunham M.~M., Lee K.~I., Arce H.~G., Fielding D.~B., 2016, ApJL, 827, L11. doi:10.3847/2041-8205/827/1/L11
\bibitem[\protect\citeauthoryear{Offner \& Chaban}{2017}]{Off17} Offner S.~S.~R., Chaban J., 2017, ApJ, 847, 104. doi:10.3847/1538-4357/aa8996
\bibitem[\protect\citeauthoryear{Offner et al.}{2022}]{Off22} Offner S.~S.~R., Taylor J., Markey C., Chen H.~H.-H., Pineda J.~E., Goodman A.~A., Burkert A., et al., 2022, MNRAS, 517, 885. doi:10.1093/mnras/stac2734
\bibitem[\protect\citeauthoryear{Ossenkopf \& Henning}{1994}]{Oss94} Ossenkopf V., Henning T., 1994, A\&A, 291, 943
\bibitem[\protect\citeauthoryear{Padoan et al.}{2020}]{Pad20} Padoan P., Pan L., Juvela M., Haugb{\o}lle T., Nordlund {\r{A}}., 2020, ApJ, 900, 82. doi:10.3847/1538-4357/abaa47
\bibitem[\protect\citeauthoryear{Peretto et al.}{2013}]{Per13} Peretto N., Fuller G.~A., Duarte-Cabral A., Avison A., Hennebelle P., Pineda J.~E., Andr{\'e} P., et al., 2013, A\&A, 555, A112. doi:10.1051/0004-6361/201321318
\bibitem[\protect\citeauthoryear{Ragan et al.}{2012}]{Rag12} Ragan S., Henning T., Krause O., Pitann J., Beuther H., Linz H., Tackenberg J., et al., 2012, A\&A, 547, A49. doi:10.1051/0004-6361/201219232
\bibitem[\protect\citeauthoryear{Rosolowsky et al.}{2008}]{Ros08} Rosolowsky E.~W., Pineda J.~E., Kauffmann J., Goodman A.~A., 2008, ApJ, 679, 1338. doi:10.1086/587685
\bibitem[\protect\citeauthoryear{Sabatini et al.}{2022}]{Sab22} Sabatini G., Bovino S., Sanhueza P., Morii K., Li S., Redaelli E., Zhang Q., et al., 2022, ApJ, 936, 80. doi:10.3847/1538-4357/ac83aa
\bibitem[\protect\citeauthoryear{Sanhueza et al.}{2010}]{San10} Sanhueza P., Garay G., Bronfman L., Mardones D., May J., Saito M., 2010, ApJ, 715, 18. doi:10.1088/0004-637X/715/1/18
\bibitem[\protect\citeauthoryear{Sanhueza et al.}{2017}]{San17} Sanhueza P., Jackson J.~M., Zhang Q., Guzm{\'a}n A.~E., Lu X., Stephens I.~W., Wang K., et al., 2017, ApJ, 841, 97. doi:10.3847/1538-4357/aa6ff8
\bibitem[\protect\citeauthoryear{Sanhueza et al.}{2019}]{San19} Sanhueza P., Contreras Y., Wu B., Jackson J.~M., Guzm{\'a}n A.~E., Zhang Q., Li S., et al., 2019, ApJ, 886, 102. doi:10.3847/1538-4357/ab45e9
\bibitem[\protect\citeauthoryear{Sanhueza et al.}{2021}]{San21} Sanhueza P., Girart J.~M., Padovani M., Galli D., Hull C.~L.~H., Zhang Q., Cortes P., et al., 2021, ApJL, 915, L10. doi:10.3847/2041-8213/ac081c
\bibitem[\protect\citeauthoryear{Saha et al.}{2022}]{Sah22} Saha A., Tej A., Liu H.-L., Liu T., Issac N., Lee C.~W., Garay G., et al., 2022, MNRAS, 516, 1983. doi:10.1093/mnras/stac2353
\bibitem[\protect\citeauthoryear{Sakai et al.}{2013}]{Sak13} Sakai T., Sakai N., Foster J.~B., Sanhueza P., Jackson J.~M., Kassis M., Furuya K., et al., 2013, ApJL, 775, L31. doi:10.1088/2041-8205/775/1/L31
\bibitem[\protect\citeauthoryear{Sakai et al.}{2022}]{Sak22} Sakai T., Sanhueza P., Furuya K., Tatematsu K., Li S., Aikawa Y., Lu X., et al., 2022, ApJ, 925, 144. doi:10.3847/1538-4357/ac3d2e
\bibitem[\protect\citeauthoryear{Schneider et al.}{2012}]{Sch12} Schneider N., Csengeri T., Hennemann M., Motte F., Didelon P., Federrath C., Bontemps S., et al., 2012, A\&A, 540, L11. doi:10.1051/0004-6361/201118566
\bibitem[\protect\citeauthoryear{Schneider et al.}{2020}]{Sch20} Schneider N., Simon R., Guevara C., Buchbender C., Higgins R.~D., Okada Y., Stutzki J., et al., 2020, PASP, 132, 104301. doi:10.1088/1538-3873/aba840
\bibitem[\protect\citeauthoryear{Schuller et al.}{2009}]{Sch09} Schuller F., Menten K.~M., Contreras Y., Wyrowski F., Schilke P., Bronfman L., Henning T., et al., 2009, A\&A, 504, 415. doi:10.1051/0004-6361/200811568
\bibitem[\protect\citeauthoryear{Stephens et al.}{2017}]{Ste17} Stephens I.~W., Dunham M.~M., Myers P.~C., Pokhrel R., Sadavoy S.~I., Vorobyov E.~I., Tobin J.~J., et al., 2017, ApJ, 846, 16. doi:10.3847/1538-4357/aa8262
\bibitem[\protect\citeauthoryear{Stutz \& Gould}{2016}]{Stu16} Stutz A.~M., Gould A., 2016, A\&A, 590, A2. doi:10.1051/0004-6361/201527979
\bibitem[\protect\citeauthoryear{Trevi{\~n}o-Morales et al.}{2019}]{Tre19} Trevi{\~n}o-Morales S.~P., Fuente A., S{\'a}nchez-Monge {\'A}., Kainulainen J., Didelon P., Suri S., Schneider N., et al., 2019, A\&A, 629, A81. doi:10.1051/0004-6361/201935260
\bibitem[\protect\citeauthoryear{Tafoya et al.}{2021}]{Taf21} Tafoya D., Sanhueza P., Zhang Q., Li S., Guzm{\'a}n A.~E., Silva A., de la Fuente E., et al., 2021, ApJ, 913, 131. doi:10.3847/1538-4357/abf5da
\bibitem[\protect\citeauthoryear{Tatematsu et al.}{2016}]{Tat16} Tatematsu K., Ohashi S., Sanhueza P., Nguyen Luong Q., Umemoto T., Mizuno N., 2016, PASJ, 68, 24. doi:10.1093/pasj/psw002
\bibitem[\protect\citeauthoryear{Thomasson et al.}{2022}]{Tho22} Thomasson B., Joncour I., Moraux E., Crespelle C., Motte F., Pouteau Y., Nony T., 2022, A\&A, 665, A119. doi:10.1051/0004-6361/202243275
\bibitem[\protect\citeauthoryear{Urquhart et al.}{2014}]{Urq14} Urquhart J.~S., Moore T.~J.~T., Csengeri T., Wyrowski F., Schuller F., Hoare M.~G., Lumsden S.~L., et al., 2014, MNRAS, 443, 1555. doi:10.1093/mnras/stu1207
\bibitem[\protect\citeauthoryear{V{\'a}zquez-Semadeni et al.}{2019}]{Vaz19} V{\'a}zquez-Semadeni E., Palau A., Ballesteros-Paredes J., G{\'o}mez G.~C., Zamora-Avil{\'e}s M., 2019, MNRAS, 490, 3061. doi:10.1093/mnras/stz2736
\bibitem[\protect\citeauthoryear{Verliat et al.}{2022}]{Ver22} Verliat A., Hennebelle P., Gonz{\'a}lez M., Lee Y.-N., Geen S., 2022, A\&A, 663, A6. doi:10.1051/0004-6361/202141765
\bibitem[\protect\citeauthoryear{Wang et al.}{2010}]{Wan10} Wang P., Li Z.-Y., Abel T., Nakamura F., 2010, ApJ, 709, 27. doi:10.1088/0004-637X/709/1/27
\bibitem[\protect\citeauthoryear{Wang et al.}{2011}]{Wan11} Wang K., Zhang Q., Wu Y., Zhang H., 2011, ApJ, 735, 64. doi:10.1088/0004-637X/735/1/64
\bibitem[\protect\citeauthoryear{Wang et al.}{2014}]{Wan14} Wang K., Zhang Q., Testi L., van der Tak F., Wu Y., Zhang H., Pillai T., et al., 2014, MNRAS, 439, 3275. doi:10.1093/mnras/stu127
\bibitem[\protect\citeauthoryear{Williams, de Geus, \& Blitz}{1994}]{Wil94} Williams J.~P., de Geus E.~J., Blitz L., 1994, ApJ, 428, 693. doi:10.1086/174279
\bibitem[\protect\citeauthoryear{Williams et al.}{2018}]{Wil18} Williams G.~M., Peretto N., Avison A., Duarte-Cabral A., Fuller G.~A., 2018, A\&A, 613, A11. doi:10.1051/0004-6361/201731587
\bibitem[\protect\citeauthoryear{Yuan et al.}{2018}]{Yua18} Yuan J., Li J.-Z., Wu Y., Ellingsen S.~P., Henkel C., Wang K., Liu T., et al., 2018, ApJ, 852, 12. doi:10.3847/1538-4357/aa9d40
\bibitem[\protect\citeauthoryear{Yuan et al.}{2021}]{Yua21} Yuan L., Yang J., Du F., Liu X., Zhang S., Lin Z., Sun J., et al., 2021, ApJS, 257, 51. doi:10.3847/1538-4365/ac242a
\bibitem[\protect\citeauthoryear{Zhang et al.}{2009}]{Zha09} Zhang Q., Wang Y., Pillai T., Rathborne J., 2009, ApJ, 696, 268. doi:10.1088/0004-637X/696/1/268
\bibitem[\protect\citeauthoryear{Zhou et al.}{2022}]{Zho22} Zhou J.-W., Liu T., Evans N.~J., Garay G., Goldsmith P.~F., G{\'o}mez G.~C., V{\'a}zquez-Semadeni E., et al., 2022, MNRAS.tmp. doi:10.1093/mnras/stac1735








\end{thebibliography}

